Search for gravitational-lensing signatures in the full third observing run of the LIGO-Virgo network

Gravitational lensing by massive objects along the line of sight to the source causes distortions of gravitational wave-signals; such distortions may reveal information about fundamental physics, cosmology and astrophysics. In this work, we have extended the search for lensing signatures to all binary black hole events from the third observing run of the LIGO--Virgo network. We search for repeated signals from strong lensing by 1) performing targeted searches for subthreshold signals, 2) calculating the degree of overlap amongst the intrinsic parameters and sky location of pairs of signals, 3) comparing the similarities of the spectrograms amongst pairs of signals, and 4) performing dual-signal Bayesian analysis that takes into account selection effects and astrophysical knowledge. We also search for distortions to the gravitational waveform caused by 1) frequency-independent phase shifts in strongly lensed images, and 2) frequency-dependent modulation of the amplitude and phase due to point masses. None of these searches yields significant evidence for lensing. Finally, we use the non-detection of gravitational-wave lensing to constrain the lensing rate based on the latest merger-rate estimates and the fraction of dark matter composed of compact objects.

==> subthreshold_combined_table.tex <==
GW$190930\_133541$ & 19-08-05 13:43:48 & $-55.994$ & 10.2 & $8.5$ & 0.002 & $61.00\%$ & $$ & $$ & $$\\
GW$191204\_171526$ & 19-08-05 13:43:48 & $-121.147$ & 10.2 & $8.55$ & 0.006 & $25.40\%$ & $$ & $$ & $$\\
GW$190425$ & 19-04-18 03:17:34 & $-7.209$ & 1.74 & $1.44$ & 0.013 & $9.49\%$ & $$ & $$ & $$\\
GW$190828\_065509$ & 19-11-12 12:13:18 & $76.221$ & 45.5 & $13.3$ & 0.023 & $18.00\%$ & $$ & $$ & $$\\
GW$200112\_155838$ & 19-04-26 19:06:42 & $-260.869$ & 28.4 & $27.4$ & 0.03 & $22.10\%$ & $$ & $$ & $$\\
GW$190725\_174728$ & 19-08-05 13:43:48 & $10.831$ & 10.2 & $7.4$ & 0.038 & $39.50\%$ & $$ & $$ & $$\\
GW$190828\_065509$ & 20-02-06 07:24:59 & $162.021$ & 15.1 & $13.3$ & 0.154 & $36.00\%$ & $$ & $$ & $$\\
GW$191103\_012549$ & 19-08-05 13:43:48 & $-89.488$ & 10.4 & $8.34$ & 0.286 & $38.00\%$ & $$ & $$ & $$\\
GW$190915\_235702$ & 19-12-10 21:44:39 & $85.908$ & 24.1 & $25.3$ & 0.301 & $21.30\%$ & $$ & $$ & $$\\
GW$191103\_012549$ & 19-12-13 16:40:18 & $40.635$ & 78.6 & $8.34$ & 0.325 & $15.40\%$ & $$ & $$ & $$\\
GW$190708\_232457$ & 19-07-07 06:08:53 & $-1.719$ & 15.4 & $13.2$ & 0.338 & $60.40\%$ & $$ & $$ & $$\\
GW$191215\_223052$ & 19-11-06 20:08:20 & $-39.099$ & 14.4 & $18.4$ & 0.35 & $28.10\%$ & $$ & $$ & $$\\
GW$191204\_171526$ & 20-03-05 10:03:54 & $91.7$ & 12.5 & $8.55$ & 0.363 & $59.80\%$ & $$ & $$ & $$\\
GW$200302\_015811$ & 19-08-19 16:55:12 & $-195.377$ & 13.6 & $23.4$ & 0.376 & $18.20\%$ & $$ & $$ & $$\\
GW$200210\_092254$ & 19-07-27 14:46:58 & $-197.775$ & 8.97 & $6.56$ & 0.426 & $29.50\%$ & $$ & $$ & $$\\
GW$191216\_213338$ & 19-08-05 13:43:48 & $-133.326$ & 10.2 & $8.33$ & 0.439 & $31.70\%$ & $$ & $$ & $$\\
GW$190425$ & 19-05-21 11:39:19 & $26.14$ & 1.49 & $1.44$ & 0.477 & $88.80\%$ & $$ & $$ & $$\\
GW$190925\_232845$ & 20-02-06 07:24:59 & $133.331$ & 15.1 & $15.8$ & 0.477 & $37.20\%$ & $$ & $$ & $$\\
GW$190426\_190642$ & 19-12-15 01:47:55 & $232.279$ & 178.0 & $77.1$ & 0.492 & $22.40\%$ & $$ & $$ & $$\\
GW$190917\_114630$ & 19-08-21 05:47:03 & $-27.25$ & 2.62 & $3.7$ & 0.521 & $51.50\%$ & $$ & $$ & $$\\
GW$191105\_143521$ & 19-11-06 20:08:20 & $1.231$ & 14.4 & $7.82$ & 0.53 & $19.90\%$ & $$ & $$ & $$\\
GW$191126\_115259$ & 19-08-24 22:43:23 & $-93.548$ & 56.8 & $8.65$ & 0.533 & $20.30\%$ & $$ & $$ & $$\\
GW$191204\_110529$ & 19-11-06 20:08:20 & $-27.623$ & 14.4 & $19.8$ & 0.546 & $19.70\%$ & $$ & $$ & $$\\
GW$191103\_012549$ & 20-01-02 03:32:57 & $60.088$ & 78.6 & $8.34$ & 0.574 & $13.10\%$ & $$ & $$ & $$\\
GW$191216\_213338$ & 20-03-13 06:37:03 & $87.377$ & 9.3 & $8.33$ & 0.628 & $33.70\%$ & $$ & $$ & $$\\
GW$190725\_174728$ & 20-02-27 18:56:18 & $217.048$ & 9.28 & $7.4$ & 0.641 & $21.60\%$ & $$ & $$ & $$\\
GW$191129\_134029$ & 20-02-11 02:33:14 & $73.537$ & 11.8 & $7.31$ & 0.704 & $7.56\%$ & $$ & $$ & $$\\
GW$200306\_093714$ & 19-12-14 10:28:27 & $-82.964$ & 17.9 & $17.5$ & 0.773 & $21.40\%$ & $$ & $$ & $$\\
GW$190725\_174728$ & 19-07-27 14:46:58 & $1.875$ & 8.56 & $7.4$ & 0.786 & $61.10\%$ & $$ & $$ & $$\\
GW$190930\_133541$ & 20-02-11 02:42:59 & $133.547$ & 9.44 & $8.5$ & 0.795 & $57.20\%$ & $$ & $$ & $$\\
GW$191103\_012549$ & 19-05-17 11:43:59 & $-169.571$ & 78.6 & $8.34$ & 0.849 & $51.20\%$ & $$ & $$ & $$\\
GW$200210\_092254$ & 20-03-05 10:03:54 & $24.028$ & 12.4 & $6.56$ & 0.88 & $3.03\%$ & $$ & $$ & $$\\
GW$191204\_171526$ & 20-02-11 02:42:59 & $68.394$ & 9.41 & $8.55$ & 0.887 & $9.15\%$ & $$ & $$ & $$\\
GW$190512\_180714$ & 20-02-06 07:24:59 & $269.554$ & 14.6 & $14.6$ & 0.944 & $0.46\%$ & $$ & $$ & $$\\
GW$190725\_174728$ & 20-02-19 19:36:34 & $209.076$ & 9.02 & $7.4$ & 1.022 & $46.10\%$ & $$ & $$ & $$\\
GW$200210\_092254$ & 20-02-01 19:49:52 & $-8.565$ & 13.7 & $6.56$ & 1.038 & $1.99\%$ & $$ & $$ & $$\\
GW$190425$ & 19-05-11 03:33:12 & $15.802$ & 1.49 & $1.44$ & 1.114 & $17.00\%$ & $$ & $$ & $$\\
GW$200210\_092254$ & 20-03-05 23:55:56 & $24.606$ & 9.63 & $6.56$ & 1.12 & $5.57\%$ & $$ & $$ & $$\\
GW$200225\_060421$ & 20-02-06 07:24:59 & $-18.944$ & 15.1 & $14.2$ & 1.127 & $10.60\%$ & $$ & $$ & $$\\
GW$190425$ & 19-09-16 15:50:27 & $144.314$ & 1.49 & $1.44$ & 1.158 & $67.30\%$ & $$ & $$ & $$\\
GW$190728\_064510$ & 20-02-27 15:28:02 & $214.363$ & 11.6 & $8.6$ & 1.199 & $32.20\%$ & $$ & $$ & $$\\
GW$190706\_222641$ & 19-08-19 16:55:12 & $43.77$ & 13.6 & $42.7$ & 1.303 & $40.20\%$ & $$ & $$ & $$\\
GW$190924\_021846$ & 19-12-25 00:57:48 & $91.944$ & 6.27 & $5.8$ & 1.303 & $100.00\%$ & $$ & $$ & $$\\
GW$190917\_114630$ & 19-11-02 08:42:03 & $45.872$ & 4.2 & $3.7$ & 1.36 & $84.60\%$ & $$ & $$ & $$\\
GW$200322\_091133$ & 20-03-19 13:50:32 & $-2.806$ & 56.1 & $15.5$ & 1.411 & $70.30\%$ & $$ & $$ & $$\\
GW$190514\_065416$ & 19-05-05 13:07:57 & $-8.74$ & 26.8 & $28.5$ & 2.361 & $13.30\%$ & $$ & $$ & $$\\
GW$190521\_074359$ & 20-01-29 18:42:35 & $253.457$ & 22.1 & $32.1$ & 1.42 & $33.60\%$ & $$ & $$ & $$\\
GW$190421\_213856$ & 19-04-18 14:48:06 & $-3.285$ & 13.6 & $31.2$ & 1.442 & $28.90\%$ & $$ & $$ & $$\\
GW$190731\_140936$ & 20-02-08 21:16:09 & $192.296$ & 33.4 & $29.5$ & 1.524 & $7.32\%$ & $$ & $$ & $$\\
GW$191126\_115259$ & 19-09-22 18:35:25 & $-64.721$ & 60.1 & $8.65$ & 1.54 & $19.40\%$ & $$ & $$ & $$\\
GW$190708\_232457$ & 19-09-09 15:12:07 & $62.658$ & 13.9 & $13.2$ & 1.581 & $37.00\%$ & $$ & $$ & $$\\
GW$191126\_115259$ & 19-08-12 01:29:34 & $-106.433$ & 44.8 & $8.65$ & 1.591 & $38.20\%$ & $$ & $$ & $$\\
GW$200210\_092254$ & 19-12-09 09:16:54 & $-63.004$ & 8.39 & $6.56$ & 1.628 & $3.82\%$ & $$ & $$ & $$\\
GW$190926\_050336$ & 19-04-26 19:06:42 & $-152.415$ & 23.8 & $25.6$ & 1.676 & $1.67\%$ & $$ & $$ & $$\\
GW$190916\_200658$ & 19-12-14 10:28:27 & $88.598$ & 33.4 & $27.3$ & 1.742 & $14.30\%$ & $$ & $$ & $$\\
GW$200306\_093714$ & 19-05-30 22:11:38 & $-280.476$ & 13.2 & $17.5$ & 1.783 & $14.60\%$ & $$ & $$ & $$\\
GW$200209\_085452$ & 19-12-26 01:48:08 & $-45.296$ & 28.4 & $26.7$ & 1.827 & $9.41\%$ & $$ & $$ & $$\\
GW$191129\_134029$ & 19-12-13 19:38:51 & $14.249$ & 8.24 & $7.31$ & 1.881 & $0.32\%$ & $$ & $$ & $$\\
GW$191126\_115259$ & 19-05-17 06:29:01 & $-193.225$ & 78.2 & $8.65$ & 1.887 & $63.10\%$ & $$ & $$ & $$\\
GW$200220\_061928$ & 19-09-03 06:51:45 & $-169.978$ & 24.9 & $62.0$ & 1.893 & $43.40\%$ & $$ & $$ & $$\\
GW$190421\_213856$ & 19-12-14 10:28:27 & $236.534$ & 29.8 & $31.2$ & 1.903 & $42.50\%$ & $$ & $$ & $$\\
GW$200302\_015811$ & 20-01-29 18:42:35 & $-32.303$ & 22.1 & $23.4$ & 1.985 & $18.80\%$ & $$ & $$ & $$\\
GW$191222\_033537$ & 19-12-14 10:28:27 & $-7.713$ & 33.4 & $33.8$ & 2.01 & $10.60\%$ & $$ & $$ & $$\\
GW$190521\_074359$ & 19-09-03 06:51:45 & $104.964$ & 21.2 & $32.1$ & 2.017 & $58.60\%$ & $$ & $$ & $$\\
GW$200225\_060421$ & 20-01-15 05:19:44 & $-41.031$ & 17.5 & $14.2$ & 2.051 & $32.80\%$ & $$ & $$ & $$\\
GW$191129\_134029$ & 19-09-25 14:52:51 & $-64.95$ & 7.78 & $7.31$ & 2.095 & $28.40\%$ & $$ & $$ & $$\\
GW$200308\_173609$ & 19-05-30 22:11:38 & $-282.809$ & 13.5 & $19.0$ & 2.13 & $46.80\%$ & $$ & $$ & $$\\
GW$190725\_174728$ & 19-11-26 11:54:01 & $123.755$ & 6.79 & $7.4$ & 2.162 & $11.20\%$ & $$ & $$ & $$\\
GW$190413\_134308$ & 20-01-10 21:46:26 & $272.336$ & 82.1 & $33.0$ & 2.177 & $37.00\%$ & $$ & $$ & $$\\
GW$190514\_065416$ & 19-07-22 06:45:25 & $68.994$ & 26.8 & $28.5$ & 3.023 & $45.40\%$ & $$ & $$ & $$\\
GW$190707\_093326$ & 19-07-03 12:03:53 & $-3.896$ & 10.4 & $8.5$ & 2.19 & $66.50\%$ & $$ & $$ & $$\\
GW$191126\_115259$ & 19-12-04 13:48:29 & $8.08$ & 78.2 & $8.65$ & 2.304 & $29.10\%$ & $$ & $$ & $$\\
GW$190517\_055101$ & 19-12-07 05:00:23 & $203.965$ & 20.3 & $26.6$ & 2.316 & $46.90\%$ & $$ & $$ & $$\\
GW$190916\_200658$ & 19-04-18 14:48:06 & $-151.221$ & 13.6 & $27.3$ & 2.319 & $34.00\%$ & $$ & $$ & $$\\
GW$190805\_211137$ & 20-01-04 18:40:28 & $151.895$ & 63.9 & $33.5$ & 2.323 & $13.40\%$ & $$ & $$ & $$\\
GW$190517\_055101$ & 19-09-03 06:51:45 & $109.042$ & 21.2 & $26.6$ & 2.338 & $37.90\%$ & $$ & $$ & $$\\
GW$200308\_173609$ & 19-04-12 08:23:54 & $-331.384$ & 35.7 & $19.0$ & 2.383 & $87.50\%$ & $$ & $$ & $$\\
GW$200115\_042309$ & 20-03-03 06:38:48 & $48.094$ & 2.32 & $2.43$ & 2.383 & $45.40\%$ & $$ & $$ & $$\\
GW$190413\_052954$ & 19-09-03 06:51:45 & $143.057$ & 23.2 & $24.6$ & 2.402 & $12.10\%$ & $$ & $$ & $$\\
GW$190926\_050336$ & 19-08-23 02:40:20 & $-34.099$ & 10.3 & $25.6$ & 2.405 & $11.30\%$ & $$ & $$ & $$\\
GW$190805\_211137$ & 19-06-13 07:45:08 & $-53.56$ & 52.8 & $33.5$ & 2.414 & $23.90\%$ & $$ & $$ & $$\\
GW$190725\_174728$ & 19-07-01 13:38:31 & $-24.173$ & 22.0 & $7.4$ & 2.433 & $18.50\%$ & $$ & $$ & $$\\
GW$200208\_130117$ & 19-09-03 06:51:45 & $-158.257$ & 21.6 & $27.7$ & 2.439 & $100.00\%$ & $$ & $$ & $$\\
GW$191113\_071753$ & 20-02-06 07:24:59 & $85.005$ & 15.3 & $10.7$ & 2.449 & $27.50\%$ & $$ & $$ & $$\\
GW$190728\_064510$ & 20-01-23 11:15:39 & $179.188$ & 9.18 & $8.6$ & 2.594 & $15.50\%$ & $$ & $$ & $$\\
GW$191129\_134029$ & 20-03-03 03:05:29 & $94.559$ & 10.7 & $7.31$ & 2.648 & $9.10\%$ & $$ & $$ & $$\\
GW$190917\_114630$ & 20-03-21 15:59:16 & $186.176$ & 2.62 & $3.7$ & 2.692 & $10.40\%$ & $$ & $$ & $$\\
GW$190925\_232845$ & 20-02-29 07:44:31 & $156.344$ & 16.3 & $15.8$ & 2.704 & $10.60\%$ & $$ & $$ & $$\\
GW$190521$ & 19-08-18 23:25:44 & $89.849$ & 71.2 & $69.2$ & 2.736 & $38.90\%$ & $$ & $$ & $$\\
GW$191126\_115259$ & 19-08-30 20:41:35 & $-87.633$ & 54.4 & $8.65$ & 2.739 & $21.90\%$ & $$ & $$ & $$\\
GW$191109\_010717$ & 20-01-10 21:46:26 & $62.861$ & 53.8 & $47.5$ & 2.752 & $11.60\%$ & $$ & $$ & $$\\
GW$191103\_012549$ & 19-07-27 14:46:58 & $-98.444$ & 8.97 & $8.34$ & 2.758 & $30.00\%$ & $$ & $$ & $$\\
GW$191129\_134029$ & 19-11-13 03:15:26 & $-16.434$ & 8.07 & $7.31$ & 2.758 & $5.88\%$ & $$ & $$ & $$\\
GW$200302\_015811$ & 19-11-06 20:08:20 & $-116.243$ & 14.7 & $23.4$ & 2.774 & $7.57\%$ & $$ & $$ & $$\\
GW$191215\_223052$ & 19-09-27 07:36:27 & $-79.621$ & 18.9 & $18.4$ & 2.783 & $59.60\%$ & $$ & $$ & $$\\
GW$190924\_021846$ & 19-07-21 09:35:01 & $-64.697$ & 6.61 & $5.8$ & 2.799 & $63.30\%$ & $$ & $$ & $$\\
GW$190426\_190642$ & 20-03-23 08:21:57 & $331.552$ & 104.0 & $77.1$ & 2.802 & $69.00\%$ & $$ & $$ & $$\\
GW$200308\_173609$ & 19-07-22 06:45:25 & $-230.452$ & 26.8 & $19.0$ & 2.824 & $78.70\%$ & $$ & $$ & $$\\
GW$190503\_185404$ & 19-09-03 06:51:45 & $122.498$ & 21.2 & $30.2$ & 2.831 & $97.60\%$ & $$ & $$ & $$\\
GW$191222\_033537$ & 20-03-19 13:50:32 & $88.427$ & 56.1 & $33.8$ & 2.862 & $7.24\%$ & $$ & $$ & $$\\
GW$191103\_012549$ & 19-09-19 13:16:54 & $-44.506$ & 33.0 & $8.34$ & 2.891 & $14.50\%$ & $$ & $$ & $$\\
GW$200202\_154313$ & 19-05-26 20:54:56 & $-251.784$ & 7.85 & $7.49$ & 2.894 & $100.00\%$ & $$ & $$ & $$\\
GW$190514\_065416$ & 19-09-03 06:51:45 & $111.998$ & 27.5 & $28.5$ & 4.323 & $38.70\%$ & $$ & $$ & $$\\
GW$191127\_050227$ & 20-01-29 18:42:35 & $63.57$ & 22.1 & $29.9$ & 2.938 & $5.72\%$ & $$ & $$ & $$\\
GW$190924\_021846$ & 19-04-25 02:45:04 & $-151.982$ & 6.45 & $5.8$ & 2.973 & $58.40\%$ & $$ & $$ & $$\\
GW$190708\_232457$ & 20-02-09 07:46:03 & $215.348$ & 21.6 & $13.2$ & 2.982 & $42.40\%$ & $$ & $$ & $$\\
GW$191105\_143521$ & 19-12-07 05:00:23 & $31.601$ & 20.3 & $7.82$ & 3.039 & $16.20\%$ & $$ & $$ & $$\\
GW$190719\_215514$ & 19-09-03 06:51:45 & $45.373$ & 21.2 & $23.5$ & 3.064 & $18.20\%$ & $$ & $$ & $$\\
GW$190413\_134308$ & 19-12-14 10:28:27 & $244.865$ & 31.1 & $33.0$ & 3.064 & $12.40\%$ & $$ & $$ & $$\\
GW$190731\_140936$ & 20-01-24 09:16:47 & $176.797$ & 33.4 & $29.5$ & 3.096 & $61.00\%$ & $$ & $$ & $$\\
GW$200209\_085452$ & 19-08-17 11:45:19 & $-175.882$ & 18.0 & $26.7$ & 3.112 & $17.20\%$ & $$ & $$ & $$\\
GW$191204\_110529$ & 19-12-07 05:00:23 & $2.746$ & 20.3 & $19.8$ & 3.112 & $37.20\%$ & $$ & $$ & $$\\
GW$191113\_071753$ & 19-09-20 09:09:00 & $-53.923$ & 13.8 & $10.7$ & 3.187 & $47.30\%$ & $$ & $$ & $$\\
GW$190707\_093326$ & 19-07-15 23:16:31 & $8.572$ & 10.1 & $8.5$ & 3.25 & $9.06\%$ & $$ & $$ & $$\\
GW$191215\_223052$ & 19-12-07 05:00:23 & $-8.729$ & 20.3 & $18.4$ & 3.25 & $12.50\%$ & $$ & $$ & $$\\
GW$190828\_065509$ & 20-03-19 17:49:16 & $204.454$ & 18.5 & $13.3$ & 3.25 & $99.80\%$ & $$ & $$ & $$\\
GW$190814$ & 19-08-22 03:35:21 & $7.267$ & 6.82 & $6.09$ & 3.282 & $100.00\%$ & $$ & $$ & $$\\
GW$190917\_114630$ & 19-09-19 18:35:06 & $2.284$ & 2.62 & $3.7$ & 3.282 & $49.10\%$ & $$ & $$ & $$\\
GW$191219\_163120$ & 20-03-23 06:48:31 & $94.595$ & 4.89 & $4.32$ & 3.282 & $79.90\%$ & $$ & $$ & $$\\
GW$191109\_010717$ & 19-08-18 23:25:44 & $-82.071$ & 78.9 & $47.5$ & 3.314 & $0.56\%$ & $$ & $$ & $$\\
GW$191230\_180458$ & 19-08-18 23:25:44 & $-133.777$ & 63.0 & $36.5$ & 3.345 & $0.54\%$ & $$ & $$ & $$\\
GW$190602\_175927$ & 20-01-04 18:40:28 & $216.028$ & 61.2 & $49.1$ & 3.408 & $21.80\%$ & $$ & $$ & $$\\
GW$200220\_061928$ & 20-01-04 18:40:28 & $-46.485$ & 56.1 & $62.0$ & 3.44 & $19.80\%$ & $$ & $$ & $$\\
GW$191204\_171526$ & 20-02-22 19:43:23 & $80.103$ & 12.2 & $8.55$ & 3.471 & $58.00\%$ & $$ & $$ & $$\\
GW$190512\_180714$ & 20-02-23 02:14:41 & $286.339$ & 12.2 & $14.6$ & 3.503 & $17.70\%$ & $$ & $$ & $$\\
GW$191129\_134029$ & 19-11-05 22:51:16 & $-23.618$ & 7.78 & $7.31$ & 3.503 & $80.00\%$ & $$ & $$ & $$\\
GW$200112\_155838$ & 19-09-03 06:51:45 & $-131.38$ & 21.2 & $27.4$ & 3.534 & $35.60\%$ & $$ & $$ & $$\\
GW$200220\_124850$ & 20-01-16 05:08:59 & $-35.319$ & 14.4 & $28.2$ & 3.534 & $94.20\%$ & $$ & $$ & $$\\
GW$200216\_220804$ & 20-02-01 13:41:54 & $-15.352$ & 13.8 & $32.9$ & 3.534 & $48.40\%$ & $$ & $$ & $$\\
GW$190521$ & 20-01-26 19:31:04 & $250.687$ & 14.7 & $69.2$ & 3.598 & $34.72\%$ & $$ & $$ & $$\\
GW$190828\_063405$ & 19-09-03 06:51:45 & $6.012$ & 21.2 & $25.0$ & 3.629 & $100.00\%$ & $$ & $$ & $$\\
GW$190910\_112807$ & 19-09-03 06:51:45 & $-7.192$ & 19.8 & $34.3$ & 3.661 & $38.40\%$ & $$ & $$ & $$\\
GW$191126\_115259$ & 20-01-16 12:36:00 & $51.03$ & 10.5 & $8.65$ & 3.661 & $6.14\%$ & $$ & $$ & $$\\
GW$190521\_074359$ & 20-01-24 09:16:47 & $248.064$ & 33.4 & $32.1$ & 3.661 & $98.40\%$ & $$ & $$ & $$\\
GW$191129\_134029$ & 19-09-21 22:57:49 & $-68.613$ & 8.6 & $7.31$ & 3.661 & $7.25\%$ & $$ & $$ & $$\\
GW$190514\_065416$ & 20-01-04 18:40:28 & $235.49$ & 56.1 & $28.5$ & 5.396 & $5.76\%$ & $$ & $$ & $$\\
GW$190706\_222641$ & 19-04-18 14:48:06 & $-79.318$ & 19.6 & $42.7$ & 3.724 & $37.30\%$ & $$ & $$ & $$\\
GW$191219\_163120$ & 19-08-21 04:58:10 & $-120.481$ & 4.73 & $4.32$ & 3.787 & $25.50\%$ & $$ & $$ & $$\\
GW$190929\_012149$ & 19-04-18 14:48:06 & $-163.44$ & 17.0 & $35.8$ & 3.85 & $8.47\%$ & $$ & $$ & $$\\
GW$190930\_133541$ & 19-11-18 11:32:17 & $48.914$ & 14.0 & $8.5$ & 3.85 & $0.32\%$ & $$ & $$ & $$\\
GW$190828\_065509$ & 20-01-30 09:59:58 & $155.128$ & 9.67 & $13.3$ & 3.945 & $0.48\%$ & $$ & $$ & $$\\
GW$191126\_115259$ & 20-01-31 13:08:37 & $66.053$ & 78.2 & $8.65$ & 3.945 & $77.10\%$ & $$ & $$ & $$\\
GW$190527\_092055$ & 20-02-08 21:16:09 & $257.497$ & 22.1 & $24.3$ & 3.945 & $3.98\%$ & $$ & $$ & $$\\
GW$190527\_092055$ & 19-09-03 06:51:45 & $98.896$ & 21.2 & $24.3$ & 3.976 & $23.60\%$ & $$ & $$ & $$\\
GW$200219\_094415$ & 19-09-03 06:51:45 & $-169.12$ & 23.2 & $27.6$ & 4.008 & $4.83\%$ & $$ & $$ & $$\\
GW$200209\_085452$ & 20-03-19 13:50:32 & $39.205$ & 48.2 & $26.7$ & 4.008 & $0.96\%$ & $$ & $$ & $$\\
GW$191129\_134029$ & 19-06-26 12:19:23 & $-156.056$ & 7.78 & $7.31$ & 4.039 & $8.44\%$ & $$ & $$ & $$\\
GW$191129\_134029$ & 19-04-03 15:42:42 & $-239.915$ & 7.78 & $7.31$ & 4.039 & $12.00\%$ & $$ & $$ & $$\\
GW$190926\_050336$ & 19-09-03 06:51:45 & $-22.925$ & 24.9 & $25.6$ & 4.071 & $78.80\%$ & $$ & $$ & $$\\
GW$190917\_114630$ & 19-07-28 18:22:16 & $-50.725$ & 2.62 & $3.7$ & 4.102 & $33.90\%$ & $$ & $$ & $$\\
GW$190707\_093326$ & 19-08-20 04:26:01 & $43.787$ & 13.3 & $8.5$ & 4.102 & $41.80\%$ & $$ & $$ & $$\\
GW$190708\_232457$ & 19-09-08 15:26:07 & $61.667$ & 14.0 & $13.2$ & 4.102 & $5.83\%$ & $$ & $$ & $$\\
GW$200112\_155838$ & 19-08-19 16:55:12 & $-145.961$ & 15.5 & $27.4$ & 4.134 & $8.42\%$ & $$ & $$ & $$\\
GW$191215\_223052$ & 20-03-03 07:41:25 & $78.382$ & 17.6 & $18.4$ & 4.134 & $18.20\%$ & $$ & $$ & $$\\
GW$200115\_042309$ & 19-04-25 06:40:59 & $-264.904$ & 2.55 & $2.43$ & 4.229 & $59.20\%$ & $$ & $$ & $$\\
GW$200112\_155838$ & 19-12-14 10:28:27 & $-29.229$ & 16.3 & $27.4$ & 4.229 & $13.40\%$ & $$ & $$ & $$\\
GW$190925\_232845$ & 19-12-31 02:46:39 & $96.137$ & 12.9 & $15.8$ & 4.229 & $28.00\%$ & $$ & $$ & $$\\
GW$191129\_134029$ & 19-06-06 06:12:30 & $-176.311$ & 8.25 & $7.31$ & 4.323 & $0.10\%$ & $$ & $$ & $$\\
GW$190924\_021846$ & 19-06-02 02:50:38 & $-113.978$ & 6.27 & $5.8$ & 4.355 & $28.90\%$ & $$ & $$ & $$\\
GW$190916\_200658$ & 20-02-08 21:16:09 & $145.048$ & 33.4 & $27.3$ & 4.355 & $8.36\%$ & $$ & $$ & $$\\
GW$190513\_205428$ & 19-09-03 06:51:45 & $112.415$ & 21.2 & $21.6$ & 4.418 & $14.60\%$ & $$ & $$ & $$\\
GW$191127\_050227$ & 19-11-10 11:42:23 & $-16.722$ & 14.5 & $29.9$ & 4.418 & $9.22\%$ & $$ & $$ & $$\\
GW$200308\_173609$ & 20-01-24 09:16:47 & $-44.347$ & 33.4 & $19.0$ & 4.45 & $73.50\%$ & $$ & $$ & $$\\
GW$191126\_115259$ & 20-02-29 06:10:57 & $94.762$ & 51.5 & $8.65$ & 4.481 & $99.30\%$ & $$ & $$ & $$\\
GW$191216\_213338$ & 19-12-14 21:28:16 & $-2.004$ & 9.67 & $8.33$ & 4.544 & $29.80\%$ & $$ & $$ & $$\\
GW$191126\_115259$ & 19-04-28 14:36:06 & $-211.887$ & 56.8 & $8.65$ & 4.576 & $41.10\%$ & $$ & $$ & $$\\
GW$190706\_222641$ & 19-08-18 23:25:44 & $43.041$ & 58.9 & $42.7$ & 4.671 & $9.96\%$ & $$ & $$ & $$\\
GW$200112\_155838$ & 19-11-06 20:08:20 & $-66.827$ & 14.7 & $27.4$ & 4.671 & $20.90\%$ & $$ & $$ & $$\\
GW$190707\_093326$ & 20-02-02 06:07:26 & $209.857$ & 11.0 & $8.5$ & 4.702 & $14.60\%$ & $$ & $$ & $$\\
GW$190426\_190642$ & 20-01-30 08:58:27 & $278.578$ & 73.6 & $77.1$ & 4.86 & $90.40\%$ & $$ & $$ & $$\\
GW$190805\_211137$ & 19-12-14 10:28:27 & $130.553$ & 26.2 & $33.5$ & 4.891 & $19.40\%$ & $$ & $$ & $$\\
GW$190803\_022701$ & 19-09-03 06:51:45 & $31.184$ & 21.6 & $27.3$ & 4.923 & $18.60\%$ & $$ & $$ & $$\\
GW$191103\_012549$ & 20-03-05 15:31:19 & $123.587$ & 13.0 & $8.34$ & 4.923 & $16.60\%$ & $$ & $$ & $$\\
GW$190620\_030421$ & 20-03-19 13:50:32 & $273.449$ & 56.1 & $38.3$ & 4.955 & $51.40\%$ & $$ & $$ & $$\\
GW$190917\_114630$ & 19-04-01 19:47:01 & $-168.666$ & 4.14 & $3.7$ & 5.018 & $8.25\%$ & $$ & $$ & $$\\
GW$190916\_200658$ & 19-08-17 11:45:19 & $-30.348$ & 18.0 & $27.3$ & 5.049 & $3.10\%$ & $$ & $$ & $$\\
GW$191129\_134029$ & 19-08-04 23:39:06 & $-116.584$ & 7.78 & $7.31$ & 5.049 & $69.60\%$ & $$ & $$ & $$\\
GW$190707\_093326$ & 19-04-03 06:58:38 & $-95.107$ & 9.92 & $8.5$ & 5.081 & $7.63\%$ & $$ & $$ & $$\\
GW$191230\_180458$ & 20-02-01 19:27:56 & $33.058$ & 20.5 & $36.5$ & 5.112 & $3.94\%$ & $$ & $$ & $$\\
GW$190425$ & 19-12-14 21:40:22 & $233.557$ & 1.49 & $1.44$ & 5.144 & $41.90\%$ & $$ & $$ & $$\\
GW$191222\_033537$ & 19-09-03 06:51:45 & $-109.864$ & 23.2 & $33.8$ & 5.175 & $29.50\%$ & $$ & $$ & $$\\
GW$191126\_115259$ & 19-09-04 06:30:53 & $-83.224$ & 60.1 & $8.65$ & 5.207 & $16.60\%$ & $$ & $$ & $$\\
GW$200306\_093714$ & 19-08-05 09:31:06 & $-214.004$ & 37.6 & $17.5$ & 5.239 & $6.13\%$ & $$ & $$ & $$\\
GW$190930\_133541$ & 19-08-23 01:13:32 & $-38.515$ & 13.2 & $8.5$ & 5.239 & $42.70\%$ & $$ & $$ & $$\\
GW$200225\_060421$ & 19-12-31 02:46:39 & $-56.137$ & 12.9 & $14.2$ & 5.239 & $43.50\%$ & $$ & $$ & $$\\
GW$200219\_094415$ & 20-01-04 18:40:28 & $-45.628$ & 54.0 & $27.6$ & 5.27 & $16.80\%$ & $$ & $$ & $$\\
GW$191129\_134029$ & 20-03-14 09:40:45 & $105.834$ & 8.38 & $7.31$ & 5.27 & $24.10\%$ & $$ & $$ & $$\\
GW$200224\_222234$ & 19-09-03 06:51:45 & $-174.646$ & 21.2 & $31.1$ & 5.302 & $43.40\%$ & $$ & $$ & $$\\
GW$200220\_061928$ & 19-09-07 21:28:02 & $-165.369$ & 12.3 & $62.0$ & 5.333 & $26.00\%$ & $$ & $$ & $$\\
GW$191219\_163120$ & 20-03-19 05:40:46 & $90.548$ & 3.42 & $4.32$ & 5.365 & $25.50\%$ & $$ & $$ & $$\\
GW$200220\_124850$ & 20-01-12 11:29:22 & $-39.055$ & 51.5 & $28.2$ & 5.396 & $67.90\%$ & $$ & $$ & $$\\
GW$190708\_232457$ & 20-01-31 12:29:29 & $206.545$ & 20.8 & $13.2$ & 5.428 & $48.40\%$ & $$ & $$ & $$\\
GW$191113\_071753$ & 19-04-08 12:06:29 & $-218.8$ & 12.9 & $10.7$ & 5.459 & $30.60\%$ & $$ & $$ & $$\\
GW$200112\_155838$ & 19-06-29 15:52:28 & $-197.004$ & 20.9 & $27.4$ & 5.459 & $0.18\%$ & $$ & $$ & $$\\
GW$190513\_205428$ & 19-12-14 10:28:27 & $214.565$ & 18.8 & $21.6$ & 5.491 & $65.60\%$ & $$ & $$ & $$\\
GW$200210\_092254$ & 19-05-11 01:05:37 & $-275.345$ & 7.53 & $6.56$ & 5.554 & $84.30\%$ & $$ & $$ & $$\\
GW$190731\_140936$ & 19-06-29 21:15:45 & $-31.704$ & 17.7 & $29.5$ & 5.617 & $6.09\%$ & $$ & $$ & $$\\
GW$200225\_060421$ & 19-07-22 06:45:25 & $-217.971$ & 26.8 & $14.2$ & 5.617 & $15.70\%$ & $$ & $$ & $$\\
GW$191103\_012549$ & 19-08-13 12:50:24 & $-81.525$ & 78.6 & $8.34$ & 5.617 & $20.70\%$ & $$ & $$ & $$\\
GW$191230\_180458$ & 20-03-01 07:54:26 & $61.576$ & 45.7 & $36.5$ & 5.617 & $100.00\%$ & $$ & $$ & $$\\
GW$190421\_213856$ & 19-09-03 06:51:45 & $134.384$ & 27.5 & $31.2$ & 5.649 & $58.30\%$ & $$ & $$ & $$\\
GW$190620\_030421$ & 19-12-14 10:28:27 & $177.308$ & 28.9 & $38.3$ & 5.649 & $32.50\%$ & $$ & $$ & $$\\
GW$190527\_092055$ & 19-12-29 02:48:23 & $215.727$ & 28.2 & $24.3$ & 5.649 & $6.79\%$ & $$ & $$ & $$\\
GW$190403\_051519$ & 20-03-15 23:18:23 & $347.752$ & 39.4 & $36.3$ & 5.649 & $9.08\%$ & $$ & $$ & $$\\
GW$191129\_134029$ & 19-05-03 14:01:51 & $-209.985$ & 7.78 & $7.31$ & 5.649 & $34.30\%$ & $$ & $$ & $$\\
GW$191103\_012549$ & 19-04-01 19:01:50 & $-215.267$ & 54.3 & $8.34$ & 5.68 & $14.50\%$ & $$ & $$ & $$\\
GW$200224\_222234$ & 19-04-18 14:48:06 & $-312.316$ & 13.6 & $31.1$ & 5.68 & $100.00\%$ & $$ & $$ & $$\\
GW$190413\_134308$ & 19-08-18 23:25:44 & $127.405$ & 87.7 & $33.0$ & 5.712 & $13.60\%$ & $$ & $$ & $$\\
GW$200220\_061928$ & 20-03-06 21:35:56 & $15.636$ & 17.4 & $62.0$ & 5.712 & $24.40\%$ & $$ & $$ & $$\\
GW$200316\_215756$ & 20-01-08 11:30:43 & $-68.436$ & 16.3 & $8.75$ & 5.775 & $84.70\%$ & $$ & $$ & $$\\
GW$191129\_134029$ & 19-08-12 08:10:12 & $-109.229$ & 7.78 & $7.31$ & 5.775 & $71.30\%$ & $$ & $$ & $$\\
GW$190403\_051519$ & 20-01-12 11:29:22 & $284.26$ & 81.7 & $36.3$ & 5.838 & $2.03\%$ & $$ & $$ & $$\\
GW$190519\_153544$ & 20-03-08 05:41:02 & $293.587$ & 19.1 & $44.5$ & 5.838 & $51.70\%$ & $$ & $$ & $$\\
GW$200308\_173609$ & 19-12-14 10:28:27 & $-85.297$ & 20.3 & $19.0$ & 5.87 & $70.90\%$ & $$ & $$ & $$\\
GW$191103\_012549$ & 20-02-11 02:42:59 & $100.054$ & 9.44 & $8.34$ & 5.87 & $43.50\%$ & $$ & $$ & $$\\
GW$191105\_143521$ & 20-03-03 07:41:25 & $118.713$ & 17.5 & $7.82$ & 5.87 & $57.60\%$ & $$ & $$ & $$\\
GW$191222\_033537$ & 19-05-05 13:07:57 & $-230.603$ & 29.6 & $33.8$ & 5.901 & $14.80\%$ & $$ & $$ & $$\\
GW$200316\_215756$ & 20-01-14 04:50:59 & $-62.713$ & 49.7 & $8.75$ & 5.933 & $83.40\%$ & $$ & $$ & $$\\
GW$190519\_153544$ & 19-04-18 14:48:06 & $-31.033$ & 17.0 & $44.5$ & 5.964 & $44.20\%$ & $$ & $$ & $$\\
GW$191204\_110529$ & 20-03-03 07:41:25 & $89.858$ & 17.5 & $19.8$ & 5.964 & $49.10\%$ & $$ & $$ & $$\\
GW$190521$ & 20-01-05 04:23:34 & $229.056$ & 13.9 & $69.2$ & 5.964 & $6.41\%$ & $$ & $$ & $$\\
GW$190924\_021846$ & 19-12-16 10:19:59 & $83.334$ & 6.33 & $5.8$ & 5.996 & $72.30\%$ & $$ & $$ & $$\\
GW$191103\_012549$ & 19-11-18 11:32:17 & $15.421$ & 14.0 & $8.34$ & 6.028 & $12.60\%$ & $$ & $$ & $$\\
GW$200129\_065458$ & 19-09-03 06:51:45 & $-148.002$ & 21.2 & $27.2$ & 6.059 & $100.00\%$ & $$ & $$ & $$\\
GW$191204\_171526$ & 19-08-17 14:35:35 & $-109.111$ & 9.7 & $8.55$ & 6.091 & $18.40\%$ & $$ & $$ & $$\\
GW$190408\_181802$ & 19-11-02 23:21:20 & $208.211$ & 23.3 & $18.3$ & 6.091 & $2.08\%$ & $$ & $$ & $$\\
GW$190521\_074359$ & 20-03-06 21:35:56 & $290.578$ & 16.7 & $32.1$ & 6.091 & $12.20\%$ & $$ & $$ & $$\\
GW$190513\_205428$ & 20-03-22 04:45:15 & $313.327$ & 18.0 & $21.6$ & 6.091 & $80.80\%$ & $$ & $$ & $$\\
GW$190706\_222641$ & 20-01-07 23:04:18 & $185.026$ & 14.3 & $42.7$ & 6.154 & $16.50\%$ & $$ & $$ & $$\\
GW$200220\_124850$ & 20-03-15 23:18:23 & $24.437$ & 37.5 & $28.2$ & 6.154 & $23.00\%$ & $$ & $$ & $$\\
GW$200306\_093714$ & 20-01-15 05:19:44 & $-51.179$ & 17.8 & $17.5$ & 6.217 & $34.70\%$ & $$ & $$ & $$\\
GW$191216\_213338$ & 19-12-08 22:32:10 & $-7.959$ & 12.0 & $8.33$ & 6.217 & $61.60\%$ & $$ & $$ & $$\\
GW$191103\_012549$ & 19-08-28 19:23:15 & $-66.252$ & 54.3 & $8.34$ & 6.248 & $28.80\%$ & $$ & $$ & $$\\
GW$190719\_215514$ & 19-12-14 10:28:27 & $147.523$ & 24.1 & $23.5$ & 6.248 & $0.83\%$ & $$ & $$ & $$\\
GW$191219\_163120$ & 19-06-21 07:55:15 & $-181.358$ & 4.71 & $4.32$ & 6.28 & $22.20\%$ & $$ & $$ & $$\\
GW$190708\_232457$ & 19-06-16 19:55:29 & $-22.145$ & 20.3 & $13.2$ & 6.312 & $43.60\%$ & $$ & $$ & $$\\
GW$190917\_114630$ & 19-11-28 11:49:41 & $72.002$ & 2.62 & $3.7$ & 6.343 & $49.60\%$ & $$ & $$ & $$\\
GW$190412$ & 19-11-16 05:23:29 & $217.995$ & 20.6 & $13.3$ & 6.375 & $9.68\%$ & $$ & $$ & $$\\
GW$190728\_064510$ & 19-04-03 06:58:38 & $-115.991$ & 9.27 & $8.6$ & 6.406 & $52.40\%$ & $$ & $$ & $$\\
GW$200302\_015811$ & 19-04-13 00:55:43 & $-324.043$ & 13.6 & $23.4$ & 6.469 & $36.50\%$ & $$ & $$ & $$\\
GW$190412$ & 19-06-16 19:55:29 & $65.601$ & 20.3 & $13.3$ & 6.469 & $30.20\%$ & $$ & $$ & $$\\
GW$190929\_012149$ & 19-09-03 06:51:45 & $-25.771$ & 19.0 & $35.8$ & 6.469 & $47.10\%$ & $$ & $$ & $$\\
GW$190929\_012149$ & 20-01-07 23:04:18 & $100.905$ & 14.3 & $35.8$ & 6.469 & $40.50\%$ & $$ & $$ & $$\\
GW$191219\_163120$ & 20-03-20 12:37:50 & $91.838$ & 4.73 & $4.32$ & 6.501 & $42.70\%$ & $$ & $$ & $$\\
GW$200210\_092254$ & 20-03-06 03:43:40 & $24.764$ & 7.74 & $6.56$ & 6.532 & $1.69\%$ & $$ & $$ & $$\\
GW$190421\_213856$ & 20-03-19 13:50:32 & $332.675$ & 49.2 & $31.2$ & 6.532 & $11.20\%$ & $$ & $$ & $$\\
GW$200210\_092254$ & 20-03-05 19:02:35 & $24.403$ & 7.66 & $6.56$ & 6.564 & $41.60\%$ & $$ & $$ & $$\\
GW$191129\_134029$ & 19-08-12 12:23:19 & $-109.054$ & 7.78 & $7.31$ & 6.564 & $18.10\%$ & $$ & $$ & $$\\
GW$191216\_213338$ & 20-03-23 19:54:26 & $97.931$ & 10.0 & $8.33$ & 6.564 & $98.70\%$ & $$ & $$ & $$\\
GW$190924\_021846$ & 20-01-29 18:46:54 & $127.686$ & 6.64 & $5.8$ & 6.596 & $49.90\%$ & $$ & $$ & $$\\
GW$191129\_134029$ & 20-02-22 06:01:36 & $84.681$ & 7.78 & $7.31$ & 6.596 & $15.00\%$ & $$ & $$ & $$\\
GW$191230\_180458$ & 20-01-04 18:40:28 & $5.025$ & 58.2 & $36.5$ & 6.596 & $75.50\%$ & $$ & $$ & $$\\
GW$190413\_052954$ & 19-08-18 23:25:44 & $127.747$ & 28.7 & $24.6$ & 6.627 & $0.10\%$ & $$ & $$ & $$\\
GW$200220\_124850$ & 19-06-20 22:22:52 & $-244.601$ & 14.4 & $28.2$ & 6.659 & $3.49\%$ & $$ & $$ & $$\\
GW$190728\_064510$ & 19-11-23 06:02:43 & $117.971$ & 9.76 & $8.6$ & 6.659 & $17.70\%$ & $$ & $$ & $$\\
GW$190916\_200658$ & 20-01-24 09:16:47 & $129.548$ & 33.4 & $27.3$ & 6.659 & $87.60\%$ & $$ & $$ & $$\\
GW$190929\_012149$ & 20-03-06 21:35:56 & $159.843$ & 14.6 & $35.8$ & 6.659 & $14.00\%$ & $$ & $$ & $$\\
GW$190924\_021846$ & 19-06-12 08:55:11 & $-103.725$ & 6.55 & $5.8$ & 6.722 & $100.00\%$ & $$ & $$ & $$\\
GW$200302\_015811$ & 19-09-03 06:51:45 & $-180.796$ & 21.2 & $23.4$ & 6.722 & $44.50\%$ & $$ & $$ & $$\\
GW$190421\_213856$ & 20-02-08 21:16:09 & $292.984$ & 28.9 & $31.2$ & 6.722 & $38.50\%$ & $$ & $$ & $$\\
GW$190708\_232457$ & 20-02-28 15:43:31 & $234.68$ & 14.6 & $13.2$ & 6.722 & $68.00\%$ & $$ & $$ & $$\\
GW$200219\_094415$ & 20-03-19 02:27:28 & $28.697$ & 54.0 & $27.6$ & 6.722 & $14.90\%$ & $$ & $$ & $$\\
GW$191105\_143521$ & 20-01-26 13:52:03 & $81.97$ & 11.9 & $7.82$ & 6.753 & $14.70\%$ & $$ & $$ & $$\\
GW$200322\_091133$ & 19-11-03 12:34:35 & $-139.859$ & 22.8 & $15.5$ & 6.816 & $70.60\%$ & $$ & $$ & $$\\
GW$191216\_213338$ & 20-01-29 17:08:30 & $43.816$ & 9.55 & $8.33$ & 6.816 & $55.20\%$ & $$ & $$ & $$\\
GW$190924\_021846$ & 19-05-26 20:55:34 & $-120.224$ & 6.27 & $5.8$ & 6.943 & $25.90\%$ & $$ & $$ & $$\\
GW$200216\_220804$ & 20-01-04 18:40:28 & $-43.144$ & 56.1 & $32.9$ & 6.943 & $10.20\%$ & $$ & $$ & $$\\
GW$200128\_022011$ & 19-04-18 14:48:06 & $-284.481$ & 13.6 & $32.0$ & 6.974 & $13.30\%$ & $$ & $$ & $$\\
GW$190708\_232457$ & 19-06-16 08:34:46 & $-22.618$ & 13.7 & $13.2$ & 6.974 & $31.20\%$ & $$ & $$ & $$\\
GW$190706\_222641$ & 19-09-15 13:44:09 & $70.637$ & 18.8 & $42.7$ & 7.037 & $12.00\%$ & $$ & $$ & $$\\
GW$190719\_215514$ & 19-09-15 13:44:09 & $57.659$ & 20.3 & $23.5$ & 7.1 & $12.80\%$ & $$ & $$ & $$\\
GW$190719\_215514$ & 20-02-08 21:16:09 & $203.973$ & 28.9 & $23.5$ & 7.132 & $0.48\%$ & $$ & $$ & $$\\
GW$190620\_030421$ & 20-03-08 05:41:02 & $262.109$ & 17.0 & $38.3$ & 7.132 & $39.00\%$ & $$ & $$ & $$\\
GW$190521\_074359$ & 19-12-14 03:05:57 & $206.807$ & 19.3 & $32.1$ & 7.164 & $50.40\%$ & $$ & $$ & $$\\
GW$190514\_065416$ & 20-02-02 18:12:25 & $264.471$ & 26.8 & $28.5$ & 9.562 & $57.40\%$ & $$ & $$ & $$\\
GW$190924\_021846$ & 19-07-10 22:07:43 & $-75.174$ & 6.27 & $5.8$ & 7.195 & $67.30\%$ & $$ & $$ & $$\\
GW$190828\_065509$ & 19-12-31 02:46:39 & $124.827$ & 13.2 & $13.3$ & 7.195 & $98.00\%$ & $$ & $$ & $$\\
GW$200322\_091133$ & 19-06-08 10:17:38 & $-287.954$ & 13.6 & $15.5$ & 7.29 & $66.90\%$ & $$ & $$ & $$\\
GW$190925\_232845$ & 19-06-21 06:01:57 & $-96.727$ & 14.4 & $15.8$ & 7.29 & $10.00\%$ & $$ & $$ & $$\\
GW$190803\_022701$ & 19-12-24 05:47:23 & $143.139$ & 24.9 & $27.3$ & 7.29 & $44.20\%$ & $$ & $$ & $$\\
GW$190916\_200658$ & 19-08-18 23:25:44 & $-28.862$ & 59.2 & $27.3$ & 7.321 & $22.30\%$ & $$ & $$ & $$\\
GW$190412$ & 20-02-09 07:46:03 & $303.094$ & 22.0 & $13.3$ & 7.321 & $64.70\%$ & $$ & $$ & $$\\
GW$190917\_114630$ & 19-11-07 04:23:07 & $50.692$ & 4.32 & $3.7$ & 7.384 & $53.30\%$ & $$ & $$ & $$\\
GW$191129\_134029$ & 19-12-21 02:34:02 & $21.537$ & 7.78 & $7.31$ & 7.384 & $88.30\%$ & $$ & $$ & $$\\
GW$190421\_213856$ & 20-01-24 09:16:47 & $277.485$ & 33.4 & $31.2$ & 7.448 & $12.70\%$ & $$ & $$ & $$\\
GW$190413\_134308$ & 20-02-18 13:24:18 & $310.987$ & 13.2 & $33.0$ & 7.479 & $50.40\%$ & $$ & $$ & $$\\
GW$191129\_134029$ & 19-11-20 09:58:40 & $-9.154$ & 7.78 & $7.31$ & 7.479 & $53.80\%$ & $$ & $$ & $$\\
GW$190707\_093326$ & 19-04-18 02:58:12 & $-80.274$ & 10.1 & $8.5$ & 7.511 & $1.44\%$ & $$ & $$ & $$\\
GW$200306\_093714$ & 20-01-13 07:06:52 & $-53.104$ & 51.1 & $17.5$ & 7.511 & $9.15\%$ & $$ & $$ & $$\\
GW$190413\_134308$ & 20-03-06 21:35:56 & $328.328$ & 16.7 & $33.0$ & 7.511 & $0.08\%$ & $$ & $$ & $$\\
GW$200220\_124850$ & 20-03-15 17:05:29 & $24.178$ & 18.8 & $28.2$ & 7.542 & $45.40\%$ & $$ & $$ & $$\\
GW$191103\_012549$ & 19-09-26 13:30:40 & $-37.497$ & 78.6 & $8.34$ & 7.574 & $39.30\%$ & $$ & $$ & $$\\
GW$191219\_163120$ & 20-01-03 19:50:12 & $15.138$ & 4.71 & $4.32$ & 7.574 & $1.83\%$ & $$ & $$ & $$\\
GW$191105\_143521$ & 20-01-28 11:54:58 & $83.889$ & 17.6 & $7.82$ & 7.574 & $24.70\%$ & $$ & $$ & $$\\
GW$190514\_065416$ & 19-08-19 16:55:12 & $97.417$ & 14.7 & $28.5$ & 10.098 & $3.97\%$ & $$ & $$ & $$\\
GW$191109\_010717$ & 20-03-15 23:18:23 & $127.924$ & 82.9 & $47.5$ & 7.7 & $21.50\%$ & $$ & $$ & $$\\
GW$191129\_134029$ & 19-12-21 01:40:18 & $21.5$ & 8.24 & $7.31$ & 7.7 & $6.80\%$ & $$ & $$ & $$\\
GW$191204\_110529$ & 20-01-26 13:52:03 & $53.116$ & 11.9 & $19.8$ & 7.826 & $24.60\%$ & $$ & $$ & $$\\
GW$190926\_050336$ & 20-03-22 04:45:15 & $177.987$ & 20.5 & $25.6$ & 7.826 & $32.80\%$ & $$ & $$ & $$\\
GW$190707\_093326$ & 19-05-25 15:17:24 & $-42.761$ & 10.1 & $8.5$ & 7.858 & $18.50\%$ & $$ & $$ & $$\\
GW$190725\_174728$ & 19-12-08 22:32:10 & $136.198$ & 12.5 & $7.4$ & 7.858 & $36.30\%$ & $$ & $$ & $$\\
GW$191126\_115259$ & 19-08-28 07:37:52 & $-90.177$ & 9.75 & $8.65$ & 7.889 & $0.91\%$ & $$ & $$ & $$\\
GW$191113\_071753$ & 19-04-11 09:06:42 & $-215.924$ & 13.4 & $10.7$ & 7.921 & $14.40\%$ & $$ & $$ & $$\\
GW$190814$ & 19-11-21 22:05:56 & $99.038$ & 7.22 & $6.09$ & 7.921 & $47.90\%$ & $$ & $$ & $$\\
GW$191204\_110529$ & 20-01-28 11:54:58 & $55.034$ & 17.6 & $19.8$ & 7.921 & $8.21\%$ & $$ & $$ & $$\\
GW$200112\_155838$ & 20-03-15 23:18:23 & $63.305$ & 86.1 & $27.4$ & 7.921 & $1.73\%$ & $$ & $$ & $$\\
GW$200302\_015811$ & 20-03-08 05:41:02 & $6.155$ & 17.0 & $23.4$ & 7.984 & $16.80\%$ & $$ & $$ & $$\\
GW$190803\_022701$ & 20-01-06 13:41:23 & $156.468$ & 47.3 & $27.3$ & 8.016 & $25.50\%$ & $$ & $$ & $$\\
GW$200308\_173609$ & 19-07-09 09:54:39 & $-243.32$ & 33.3 & $19.0$ & 8.047 & $61.20\%$ & $$ & $$ & $$\\
GW$200220\_124850$ & 19-08-01 12:11:43 & $-203.026$ & 23.4 & $28.2$ & 8.047 & $11.50\%$ & $$ & $$ & $$\\
GW$190926\_050336$ & 19-08-30 20:41:32 & $-26.349$ & 18.6 & $25.6$ & 8.047 & $0.08\%$ & $$ & $$ & $$\\
GW$200220\_124850$ & 19-05-17 17:22:51 & $-278.81$ & 17.7 & $28.2$ & 8.079 & $58.50\%$ & $$ & $$ & $$\\
GW$200208\_222617$ & 20-01-16 05:08:59 & $-23.72$ & 56.1 & $19.6$ & 8.11 & $85.40\%$ & $$ & $$ & $$\\
GW$200220\_061928$ & 19-12-14 03:05:57 & $-68.134$ & 20.6 & $62.0$ & 8.142 & $55.10\%$ & $$ & $$ & $$\\
GW$191103\_012549$ & 20-03-12 14:43:11 & $130.554$ & 78.6 & $8.34$ & 8.142 & $68.00\%$ & $$ & $$ & $$\\
GW$190814$ & 19-05-03 07:20:09 & $-103.577$ & 6.29 & $6.09$ & 8.173 & $100.00\%$ & $$ & $$ & $$\\
GW$200220\_124850$ & 19-07-05 19:29:05 & $-229.722$ & 18.8 & $28.2$ & 8.173 & $7.40\%$ & $$ & $$ & $$\\
GW$190731\_140936$ & 19-09-03 06:51:45 & $33.696$ & 20.7 & $29.5$ & 8.205 & $44.40\%$ & $$ & $$ & $$\\
GW$190929\_012149$ & 19-09-07 21:28:02 & $-21.162$ & 12.3 & $35.8$ & 8.237 & $12.20\%$ & $$ & $$ & $$\\
GW$190926\_050336$ & 19-12-14 03:05:57 & $78.918$ & 19.3 & $25.6$ & 8.268 & $1.75\%$ & $$ & $$ & $$\\
GW$190917\_114630$ & 19-04-07 09:37:25 & $-163.09$ & 4.24 & $3.7$ & 8.3 & $2.75\%$ & $$ & $$ & $$\\
GW$190708\_232457$ & 20-03-08 06:32:00 & $243.297$ & 14.9 & $13.2$ & 8.331 & $30.10\%$ & $$ & $$ & $$\\
GW$190917\_114630$ & 19-04-06 07:10:39 & $-164.192$ & 2.62 & $3.7$ & 8.363 & $55.40\%$ & $$ & $$ & $$\\
GW$200322\_091133$ & 19-06-20 22:22:52 & $-275.45$ & 13.6 & $15.5$ & 8.394 & $59.00\%$ & $$ & $$ & $$\\
GW$190421\_213856$ & 20-01-04 18:40:28 & $257.876$ & 58.2 & $31.2$ & 8.394 & $5.74\%$ & $$ & $$ & $$\\
GW$190521$ & 20-03-21 18:04:34 & $305.626$ & 25.0 & $69.2$ & 8.394 & $4.92\%$ & $$ & $$ & $$\\
GW$191129\_134029$ & 20-03-14 22:37:57 & $106.373$ & 9.47 & $7.31$ & 8.394 & $0.44\%$ & $$ & $$ & $$\\
GW$200112\_155838$ & 19-12-10 13:21:17 & $-33.109$ & 26.3 & $27.4$ & 8.426 & $49.90\%$ & $$ & $$ & $$\\
GW$190917\_114630$ & 20-01-27 17:20:27 & $132.232$ & 4.24 & $3.7$ & 8.426 & $1.68\%$ & $$ & $$ & $$\\
GW$200210\_092254$ & 20-01-24 09:48:31 & $-16.982$ & 8.3 & $6.56$ & 8.457 & $47.90\%$ & $$ & $$ & $$\\
GW$190513\_205428$ & 19-08-19 16:55:12 & $97.834$ & 17.8 & $21.6$ & 8.489 & $12.20\%$ & $$ & $$ & $$\\
GW$190916\_200658$ & 20-02-02 17:01:04 & $138.871$ & 14.5 & $27.3$ & 8.489 & $39.40\%$ & $$ & $$ & $$\\
GW$191222\_033537$ & 19-09-01 00:51:13 & $-112.114$ & 15.3 & $33.8$ & 8.521 & $3.71\%$ & $$ & $$ & $$\\
GW$190425$ & 20-02-29 20:10:54 & $310.495$ & 1.49 & $1.44$ & 8.521 & $70.20\%$ & $$ & $$ & $$\\
GW$190403\_051519$ & 20-01-15 05:19:44 & $287.003$ & 16.8 & $36.3$ & 8.552 & $30.30\%$ & $$ & $$ & $$\\
GW$191129\_134029$ & 20-01-06 05:49:12 & $37.673$ & 8.25 & $7.31$ & 8.552 & $8.57\%$ & $$ & $$ & $$\\
GW$190910\_112807$ & 19-04-18 14:48:06 & $-144.861$ & 17.0 & $34.3$ & 8.584 & $24.70\%$ & $$ & $$ & $$\\
GW$190916\_200658$ & 20-03-06 21:35:56 & $172.062$ & 16.7 & $27.3$ & 8.584 & $1.91\%$ & $$ & $$ & $$\\
GW$190513\_205428$ & 19-06-25 01:48:38 & $42.204$ & 21.3 & $21.6$ & 8.615 & $25.80\%$ & $$ & $$ & $$\\
GW$190803\_022701$ & 19-06-29 21:15:45 & $-34.216$ & 17.6 & $27.3$ & 8.615 & $10.70\%$ & $$ & $$ & $$\\
GW$190917\_114630$ & 19-11-17 02:32:57 & $60.616$ & 2.62 & $3.7$ & 8.615 & $3.68\%$ & $$ & $$ & $$\\
GW$190421\_213856$ & 20-01-29 18:42:35 & $282.878$ & 22.2 & $31.2$ & 8.647 & $9.69\%$ & $$ & $$ & $$\\
GW$190926\_050336$ & 19-09-15 13:44:09 & $-10.639$ & 20.3 & $25.6$ & 8.741 & $48.10\%$ & $$ & $$ & $$\\
GW$190916\_200658$ & 20-01-03 06:05:01 & $108.415$ & 28.2 & $27.3$ & 8.741 & $24.00\%$ & $$ & $$ & $$\\
GW$200225\_060421$ & 19-08-22 09:35:17 & $-186.854$ & 12.0 & $14.2$ & 8.836 & $41.30\%$ & $$ & $$ & $$\\
GW$190519\_153544$ & 20-01-07 23:04:18 & $233.312$ & 14.3 & $44.5$ & 8.931 & $12.40\%$ & $$ & $$ & $$\\
GW$190521$ & 20-01-07 23:04:18 & $231.835$ & 13.8 & $69.2$ & 8.931 & $6.38\%$ & $$ & $$ & $$\\
GW$190630\_185205$ & 19-11-06 20:08:20 & $129.053$ & 14.7 & $24.9$ & 8.962 & $12.20\%$ & $$ & $$ & $$\\
GW$190910\_112807$ & 20-03-06 21:35:56 & $178.422$ & 17.2 & $34.3$ & 8.962 & $12.10\%$ & $$ & $$ & $$\\
GW$191204\_171526$ & 20-03-20 13:08:04 & $106.828$ & 12.6 & $8.55$ & 8.962 & $15.40\%$ & $$ & $$ & $$\\
GW$191113\_071753$ & 19-09-08 15:26:07 & $-65.661$ & 14.0 & $10.7$ & 9.025 & $17.90\%$ & $$ & $$ & $$\\
GW$190412$ & 20-02-26 12:02:12 & $320.272$ & 46.2 & $13.3$ & 9.025 & $100.00\%$ & $$ & $$ & $$\\
GW$191103\_012549$ & 20-03-23 13:53:52 & $141.519$ & 8.59 & $8.34$ & 9.025 & $15.80\%$ & $$ & $$ & $$\\
GW$190731\_140936$ & 19-09-15 13:44:09 & $45.982$ & 19.3 & $29.5$ & 9.057 & $37.20\%$ & $$ & $$ & $$\\
GW$190924\_021846$ & 19-07-04 08:43:40 & $-81.733$ & 6.27 & $5.8$ & 9.12 & $100.00\%$ & $$ & $$ & $$\\
GW$190708\_232457$ & 19-08-10 08:57:12 & $32.397$ & 20.5 & $13.2$ & 9.12 & $28.10\%$ & $$ & $$ & $$\\
GW$190930\_133541$ & 20-01-08 18:18:19 & $100.196$ & 9.74 & $8.5$ & 9.12 & $10.20\%$ & $$ & $$ & $$\\
GW$190519\_153544$ & 19-05-05 13:07:57 & $-14.103$ & 24.9 & $44.5$ & 9.183 & $45.50\%$ & $$ & $$ & $$\\
GW$190814$ & 19-06-16 09:50:28 & $-59.472$ & 6.29 & $6.09$ & 9.215 & $20.00\%$ & $$ & $$ & $$\\
GW$191126\_115259$ & 20-01-25 15:38:11 & $60.156$ & 38.2 & $8.65$ & 9.215 & $54.80\%$ & $$ & $$ & $$\\
GW$200112\_155838$ & 20-01-28 11:54:58 & $15.831$ & 18.7 & $27.4$ & 9.246 & $6.79\%$ & $$ & $$ & $$\\
GW$190929\_012149$ & 20-02-18 13:24:18 & $142.502$ & 13.2 & $35.8$ & 9.246 & $59.70\%$ & $$ & $$ & $$\\
GW$190917\_114630$ & 20-02-21 00:35:08 & $156.534$ & 4.39 & $3.7$ & 9.246 & $38.70\%$ & $$ & $$ & $$\\
GW$191216\_213338$ & 20-01-28 00:10:34 & $42.109$ & 8.72 & $8.33$ & 9.246 & $100.00\%$ & $$ & $$ & $$\\
GW$190728\_064510$ & 19-09-09 21:26:39 & $43.612$ & 10.4 & $8.6$ & 9.341 & $5.56\%$ & $$ & $$ & $$\\
GW$191126\_115259$ & 19-09-23 02:18:49 & $-64.399$ & 44.8 & $8.65$ & 9.341 & $14.00\%$ & $$ & $$ & $$\\
GW$191129\_134029$ & 19-09-19 11:09:09 & $-71.105$ & 7.78 & $7.31$ & 9.341 & $80.70\%$ & $$ & $$ & $$\\
GW$190514\_065416$ & 20-01-14 08:07:42 & $245.051$ & 26.8 & $28.5$ & 12.087 & $43.50\%$ & $$ & $$ & $$\\
GW$200209\_085452$ & 19-09-19 02:11:14 & $-143.28$ & 22.5 & $26.7$ & 9.404 & $12.10\%$ & $$ & $$ & $$\\
GW$190917\_114630$ & 20-02-21 05:23:13 & $156.734$ & 2.62 & $3.7$ & 9.404 & $15.10\%$ & $$ & $$ & $$\\
GW$191126\_115259$ & 19-05-12 15:50:08 & $-197.835$ & 51.5 & $8.65$ & 9.499 & $7.25\%$ & $$ & $$ & $$\\
GW$191113\_071753$ & 19-12-29 00:48:11 & $45.729$ & 13.2 & $10.7$ & 9.53 & $92.30\%$ & $$ & $$ & $$\\
GW$200128\_022011$ & 19-08-18 23:25:44 & $-162.121$ & 77.2 & $32.0$ & 9.594 & $10.90\%$ & $$ & $$ & $$\\
GW$191126\_115259$ & 20-03-04 13:56:10 & $99.086$ & 44.8 & $8.65$ & 9.625 & $65.00\%$ & $$ & $$ & $$\\
GW$190917\_114630$ & 19-04-22 12:28:50 & $-147.971$ & 4.21 & $3.7$ & 9.688 & $13.40\%$ & $$ & $$ & $$\\
GW$200115\_042309$ & 19-06-04 09:45:37 & $-224.776$ & 2.67 & $2.43$ & 9.688 & $12.60\%$ & $$ & $$ & $$\\
GW$190828\_065509$ & 19-11-24 22:37:45 & $88.655$ & 14.4 & $13.3$ & 9.688 & $55.00\%$ & $$ & $$ & $$\\
GW$200208\_222617$ & 19-12-14 10:28:27 & $-56.498$ & 36.0 & $19.6$ & 9.72 & $8.15\%$ & $$ & $$ & $$\\
GW$190403\_051519$ & 19-12-07 05:00:23 & $247.99$ & 20.3 & $36.3$ & 9.751 & $17.80\%$ & $$ & $$ & $$\\
GW$200129\_065458$ & 19-06-25 01:48:38 & $-218.213$ & 23.3 & $27.2$ & 9.783 & $59.80\%$ & $$ & $$ & $$\\
GW$190916\_200658$ & 19-09-03 06:51:45 & $-13.552$ & 23.9 & $27.3$ & 9.783 & $10.60\%$ & $$ & $$ & $$\\
GW$190517\_055101$ & 19-12-10 13:21:17 & $207.313$ & 26.1 & $26.6$ & 9.783 & $63.80\%$ & $$ & $$ & $$\\
GW$190917\_114630$ & 20-02-22 02:11:40 & $157.601$ & 5.45 & $3.7$ & 9.783 & $59.10\%$ & $$ & $$ & $$\\
GW$190925\_232845$ & 20-03-19 17:49:16 & $175.764$ & 18.5 & $15.8$ & 9.814 & $95.10\%$ & $$ & $$ & $$\\
GW$190708\_232457$ & 19-12-21 12:35:05 & $165.549$ & 21.8 & $13.2$ & 9.878 & $76.00\%$ & $$ & $$ & $$\\
GW$190917\_114630$ & 19-07-21 09:17:43 & $-58.103$ & 2.62 & $3.7$ & 9.941 & $66.50\%$ & $$ & $$ & $$\\
GW$190408\_181802$ & 19-06-01 20:17:54 & $54.083$ & 15.9 & $18.3$ & 10.035 & $38.10\%$ & $$ & $$ & $$\\
GW$191219\_163120$ & 19-06-29 16:16:20 & $-173.01$ & 4.73 & $4.32$ & 10.035 & $13.20\%$ & $$ & $$ & $$\\
GW$200316\_215756$ & 19-07-08 03:56:36 & $-252.751$ & 10.8 & $8.75$ & 10.035 & $85.80\%$ & $$ & $$ & $$\\
GW$190915\_235702$ & 19-09-19 02:11:14 & $3.093$ & 22.5 & $25.3$ & 10.035 & $21.70\%$ & $$ & $$ & $$\\
GW$190706\_222641$ & 19-11-17 02:52:05 & $133.184$ & 13.6 & $42.7$ & 10.067 & $0.48\%$ & $$ & $$ & $$\\
GW$190915\_235702$ & 20-03-22 04:45:15 & $188.2$ & 18.5 & $25.3$ & 10.098 & $61.50\%$ & $$ & $$ & $$\\
GW$190917\_114630$ & 19-08-26 10:36:08 & $-22.049$ & 4.28 & $3.7$ & 10.193 & $48.60\%$ & $$ & $$ & $$\\
GW$190421\_213856$ & 19-12-14 03:05:57 & $236.227$ & 20.6 & $31.2$ & 10.193 & $4.22\%$ & $$ & $$ & $$\\
GW$190426\_190642$ & 20-01-31 13:08:37 & $279.751$ & 73.6 & $77.1$ & 10.288 & $85.90\%$ & $$ & $$ & $$\\
GW$190630\_185205$ & 19-12-05 15:50:08 & $157.874$ & 13.7 & $24.9$ & 10.319 & $22.20\%$ & $$ & $$ & $$\\
GW$190708\_232457$ & 20-03-20 01:22:23 & $255.082$ & 16.8 & $13.2$ & 10.351 & $43.60\%$ & $$ & $$ & $$\\
GW$191113\_071753$ & 19-06-21 06:01:57 & $-145.053$ & 14.6 & $10.7$ & 10.382 & $1.00\%$ & $$ & $$ & $$\\
GW$200210\_092254$ & 20-02-01 07:46:30 & $-9.067$ & 7.99 & $6.56$ & 10.382 & $15.40\%$ & $$ & $$ & $$\\
GW$190707\_093326$ & 19-06-15 01:33:58 & $-22.333$ & 10.4 & $8.5$ & 10.414 & $31.10\%$ & $$ & $$ & $$\\
GW$200302\_015811$ & 19-07-26 12:49:10 & $-219.548$ & 11.3 & $23.4$ & 10.446 & $41.10\%$ & $$ & $$ & $$\\
GW$200220\_124850$ & 20-01-15 11:02:29 & $-36.074$ & 14.4 & $28.2$ & 10.446 & $41.40\%$ & $$ & $$ & $$\\
GW$191126\_115259$ & 20-02-26 00:11:48 & $91.513$ & 37.4 & $8.65$ & 10.446 & $53.80\%$ & $$ & $$ & $$\\
GW$190706\_222641$ & 19-04-13 00:55:43 & $-84.897$ & 14.2 & $42.7$ & 10.477 & $47.80\%$ & $$ & $$ & $$\\
GW$200112\_155838$ & 19-09-19 02:11:14 & $-115.575$ & 22.5 & $27.4$ & 10.477 & $26.70\%$ & $$ & $$ & $$\\
GW$190828\_065509$ & 20-02-02 16:23:18 & $158.395$ & 15.6 & $13.3$ & 10.477 & $98.00\%$ & $$ & $$ & $$\\
GW$200202\_154313$ & 20-01-29 13:16:57 & $-4.102$ & 8.87 & $7.49$ & 10.477 & $85.20\%$ & $$ & $$ & $$\\
GW$190707\_093326$ & 19-12-14 13:39:07 & $160.171$ & 9.8 & $8.5$ & 10.509 & $10.90\%$ & $$ & $$ & $$\\
GW$191216\_213338$ & 20-02-17 23:05:18 & $63.064$ & 8.77 & $8.33$ & 10.509 & $64.70\%$ & $$ & $$ & $$\\
GW$200302\_015811$ & 20-02-08 21:16:09 & $-22.196$ & 22.1 & $23.4$ & 10.54 & $25.20\%$ & $$ & $$ & $$\\
GW$190828\_065509$ & 20-03-26 15:22:16 & $211.352$ & 17.3 & $13.3$ & 10.666 & $15.20\%$ & $$ & $$ & $$\\
GW$190426\_190642$ & 20-01-04 18:40:28 & $252.982$ & 60.3 & $77.1$ & 10.73 & $41.20\%$ & $$ & $$ & $$\\
GW$200220\_124850$ & 20-03-12 09:39:03 & $20.868$ & 23.4 & $28.2$ & 10.73 & $53.70\%$ & $$ & $$ & $$\\
GW$200128\_022011$ & 19-04-12 08:23:54 & $-290.747$ & 33.6 & $32.0$ & 10.793 & $0.82\%$ & $$ & $$ & $$\\
GW$190421\_213856$ & 19-11-17 02:52:05 & $209.217$ & 13.6 & $31.2$ & 10.793 & $9.00\%$ & $$ & $$ & $$\\
GW$190706\_222641$ & 20-01-26 09:49:57 & $203.474$ & 13.7 & $42.7$ & 10.793 & $67.10\%$ & $$ & $$ & $$\\
GW$200202\_154313$ & 20-03-11 08:42:26 & $37.708$ & 7.85 & $7.49$ & 10.793 & $17.20\%$ & $$ & $$ & $$\\
GW$190602\_175927$ & 19-09-03 06:51:45 & $92.536$ & 23.7 & $49.1$ & 10.824 & $81.80\%$ & $$ & $$ & $$\\
GW$191109\_010717$ & 19-04-18 14:48:06 & $-204.43$ & 17.0 & $47.5$ & 10.856 & $3.97\%$ & $$ & $$ & $$\\
GW$191109\_010717$ & 20-03-06 21:35:56 & $118.853$ & 16.3 & $47.5$ & 10.856 & $10.50\%$ & $$ & $$ & $$\\
GW$191105\_143521$ & 20-03-15 07:07:10 & $130.689$ & 14.1 & $7.82$ & 10.919 & $96.10\%$ & $$ & $$ & $$\\
GW$191216\_213338$ & 20-02-03 04:10:06 & $48.275$ & 8.61 & $8.33$ & 10.919 & $8.01\%$ & $$ & $$ & $$\\
GW$190708\_232457$ & 19-06-16 10:17:28 & $-22.547$ & 14.4 & $13.2$ & 10.95 & $99.20\%$ & $$ & $$ & $$\\
GW$190915\_235702$ & 19-08-19 16:55:12 & $-27.293$ & 14.7 & $25.3$ & 10.95 & $19.20\%$ & $$ & $$ & $$\\
GW$190706\_222641$ & 20-01-29 06:29:48 & $206.336$ & 14.3 & $42.7$ & 10.95 & $85.10\%$ & $$ & $$ & $$\\
GW$200308\_173609$ & 19-12-29 02:48:23 & $-70.617$ & 29.1 & $19.0$ & 10.982 & $57.80\%$ & $$ & $$ & $$\\
GW$190828\_065509$ & 20-02-04 06:58:23 & $160.002$ & 17.2 & $13.3$ & 10.982 & $17.80\%$ & $$ & $$ & $$\\
GW$190708\_232457$ & 19-04-09 10:04:55 & $-90.556$ & 14.4 & $13.2$ & 11.045 & $22.80\%$ & $$ & $$ & $$\\
GW$200311_115853$ & 19-04-22 15:57:10 & $-323.835$ & 14.5 & $26.6$ & 11.045 & $100.00\%$ & $$ & $$ & $$\\
GW$190803\_022701$ & 19-12-14 03:05:57 & $133.027$ & 20.6 & $27.3$ & 11.045 & $51.40\%$ & $$ & $$ & $$\\
GW$190828\_065509$ & 19-11-24 08:31:10 & $88.067$ & 24.4 & $13.3$ & 11.077 & $0.72\%$ & $$ & $$ & $$\\
GW$191126\_115259$ & 19-12-05 07:53:05 & $8.833$ & 51.5 & $8.65$ & 11.077 & $18.70\%$ & $$ & $$ & $$\\
GW$190725\_174728$ & 20-02-01 07:46:30 & $190.583$ & 7.36 & $7.4$ & 11.077 & $45.60\%$ & $$ & $$ & $$\\
GW$190630\_185205$ & 20-02-08 21:16:09 & $223.1$ & 22.6 & $24.9$ & 11.203 & $10.30\%$ & $$ & $$ & $$\\
GW$200322\_091133$ & 20-02-14 04:36:51 & $-37.191$ & 20.7 & $15.5$ & 11.203 & $87.40\%$ & $$ & $$ & $$\\
GW$190924\_021846$ & 20-03-01 21:50:34 & $159.814$ & 6.25 & $5.8$ & 11.203 & $71.80\%$ & $$ & $$ & $$\\
GW$190517\_055101$ & 19-08-19 16:55:12 & $94.461$ & 14.7 & $26.6$ & 11.266 & $8.25\%$ & $$ & $$ & $$\\
GW$190706\_222641$ & 19-06-29 21:15:45 & $-7.049$ & 17.7 & $42.7$ & 11.298 & $19.90\%$ & $$ & $$ & $$\\
GW$190426\_190642$ & 20-02-02 03:29:33 & $281.349$ & 73.6 & $77.1$ & 11.298 & $61.60\%$ & $$ & $$ & $$\\
GW$190708\_232457$ & 19-11-02 08:55:25 & $116.396$ & 16.5 & $13.2$ & 11.329 & $36.60\%$ & $$ & $$ & $$\\
GW$200128\_022011$ & 19-09-03 06:51:45 & $-146.811$ & 21.6 & $32.0$ & 11.361 & $19.90\%$ & $$ & $$ & $$\\
GW$190706\_222641$ & 19-07-03 12:00:34 & $-3.435$ & 16.9 & $42.7$ & 11.455 & $0.99\%$ & $$ & $$ & $$\\
GW$190620\_030421$ & 19-09-03 06:51:45 & $75.158$ & 20.8 & $38.3$ & 11.455 & $23.40\%$ & $$ & $$ & $$\\
GW$191215\_223052$ & 20-03-25 02:37:54 & $100.172$ & 18.9 & $18.4$ & 11.455 & $9.85\%$ & $$ & $$ & $$\\
GW$200115\_042309$ & 19-08-05 02:41:02 & $-163.071$ & 2.32 & $2.43$ & 11.487 & $87.90\%$ & $$ & $$ & $$\\
GW$191127\_050227$ & 19-09-03 06:51:45 & $-84.924$ & 21.2 & $29.9$ & 11.519 & $41.80\%$ & $$ & $$ & $$\\
GW$191204\_110529$ & 20-03-15 07:07:10 & $101.834$ & 14.1 & $19.8$ & 11.519 & $62.70\%$ & $$ & $$ & $$\\
GW$200210\_092254$ & 20-02-28 10:49:28 & $18.06$ & 10.7 & $6.56$ & 11.55 & $1.20\%$ & $$ & $$ & $$\\
GW$191215\_223052$ & 19-11-07 04:32:02 & $-38.749$ & 19.6 & $18.4$ & 11.582 & $3.08\%$ & $$ & $$ & $$\\
GW$200216\_220804$ & 19-06-05 02:59:57 & $-256.797$ & 79.3 & $32.9$ & 11.613 & $37.90\%$ & $$ & $$ & $$\\
GW$200225\_060421$ & 20-03-16 23:02:41 & $20.707$ & 28.7 & $14.2$ & 11.613 & $65.20\%$ & $$ & $$ & $$\\
GW$200216\_220804$ & 19-09-30 06:26:55 & $-139.654$ & 79.3 & $32.9$ & 11.645 & $17.60\%$ & $$ & $$ & $$\\
GW$190803\_022701$ & 20-01-16 19:04:54 & $166.693$ & 30.2 & $27.3$ & 11.645 & $3.03\%$ & $$ & $$ & $$\\
GW$191204\_110529$ & 20-03-22 04:45:15 & $108.736$ & 17.4 & $19.8$ & 11.676 & $64.40\%$ & $$ & $$ & $$\\
GW$200208\_222617$ & 20-02-27 12:15:32 & $18.576$ & 16.9 & $19.6$ & 11.676 & $13.60\%$ & $$ & $$ & $$\\
GW$191219\_163120$ & 19-05-01 11:58:05 & $-232.19$ & 4.65 & $4.32$ & 11.739 & $0.28\%$ & $$ & $$ & $$\\
GW$191215\_223052$ & 19-06-01 20:17:54 & $-197.092$ & 16.4 & $18.4$ & 11.739 & $11.80\%$ & $$ & $$ & $$\\
GW$200220\_124850$ & 20-02-12 11:49:34 & $-8.041$ & 18.8 & $28.2$ & 11.739 & $33.20\%$ & $$ & $$ & $$\\
GW$190929\_012149$ & 20-02-11 22:39:49 & $135.888$ & 15.9 & $35.8$ & 11.771 & $6.18\%$ & $$ & $$ & $$\\
GW$200306\_093714$ & 20-01-04 18:40:28 & $-61.623$ & 56.7 & $17.5$ & 11.803 & $3.42\%$ & $$ & $$ & $$\\
GW$190708\_232457$ & 20-02-21 01:39:35 & $227.093$ & 16.0 & $13.2$ & 11.803 & $49.10\%$ & $$ & $$ & $$\\
GW$190725\_174728$ & 19-04-25 13:17:59 & $-91.187$ & 8.42 & $7.4$ & 11.834 & $7.10\%$ & $$ & $$ & $$\\
GW$191219\_163120$ & 20-01-13 18:36:35 & $25.087$ & 4.69 & $4.32$ & 11.866 & $37.30\%$ & $$ & $$ & $$\\
GW$190620\_030421$ & 19-08-18 23:25:44 & $59.848$ & 77.2 & $38.3$ & 11.897 & $32.00\%$ & $$ & $$ & $$\\
GW$190412$ & 19-04-08 12:06:29 & $-3.725$ & 12.5 & $13.3$ & 11.929 & $29.20\%$ & $$ & $$ & $$\\
GW$190706\_222641$ & 20-01-31 09:15:21 & $208.45$ & 22.0 & $42.7$ & 11.929 & $94.30\%$ & $$ & $$ & $$\\
GW$200308\_173609$ & 19-07-01 15:18:40 & $-251.095$ & 33.0 & $19.0$ & 12.055 & $75.30\%$ & $$ & $$ & $$\\
GW$190926\_050336$ & 19-12-29 02:48:23 & $93.906$ & 20.9 & $25.6$ & 12.055 & $3.16\%$ & $$ & $$ & $$\\
GW$191105\_143521$ & 19-12-29 02:48:23 & $53.509$ & 32.2 & $7.82$ & 12.055 & $3.96\%$ & $$ & $$ & $$\\
GW$200322\_091133$ & 19-05-12 00:59:07 & $-315.342$ & 26.7 & $15.5$ & 12.087 & $85.30\%$ & $$ & $$ & $$\\
GW$191204\_110529$ & 19-12-29 02:48:23 & $24.655$ & 32.2 & $19.8$ & 12.087 & $13.50\%$ & $$ & $$ & $$\\
GW$191109\_010717$ & 20-03-25 00:42:38 & $136.983$ & 14.0 & $47.5$ & 12.087 & $10.80\%$ & $$ & $$ & $$\\
GW$191215\_223052$ & 19-04-10 09:46:08 & $-249.531$ & 20.3 & $18.4$ & 12.118 & $58.60\%$ & $$ & $$ & $$\\
GW$190828\_063405$ & 19-06-25 01:48:38 & $-64.198$ & 24.4 & $25.0$ & 12.118 & $0.05\%$ & $$ & $$ & $$\\
GW$190630\_185205$ & 19-09-03 06:51:45 & $64.5$ & 24.9 & $24.9$ & 12.118 & $12.10\%$ & $$ & $$ & $$\\
GW$190426\_190642$ & 19-11-21 20:04:31 & $209.04$ & 178.0 & $77.1$ & 12.118 & $28.50\%$ & $$ & $$ & $$\\
GW$190706\_222641$ & 20-03-05 18:49:18 & $242.849$ & 13.9 & $42.7$ & 12.118 & $13.40\%$ & $$ & $$ & $$\\
GW$200306\_093714$ & 19-05-09 15:17:45 & $-301.764$ & 39.6 & $17.5$ & 12.15 & $29.60\%$ & $$ & $$ & $$\\
GW$190426\_190642$ & 19-11-02 12:46:29 & $189.736$ & 104.0 & $77.1$ & 12.15 & $35.30\%$ & $$ & $$ & $$\\

